Neural Architectures for Open-Type Relation Argument Extraction

In this work, we introduce the task of Open-Type Relation Argument Extraction (ORAE): Given a corpus, a query entity Q and a knowledge base relation (e.g.,"Q authored notable work with title X"), the model has to extract an argument of non-standard entity type (entities that cannot be extracted by a standard named entity tagger, e.g. X: the title of a book or a work of art) from the corpus. A distantly supervised dataset based on WikiData relations is obtained and released to address the task. We develop and compare a wide range of neural models for this task yielding large improvements over a strong baseline obtained with a neural question answering system. The impact of different sentence encoding architectures and answer extraction methods is systematically compared. An encoder based on gated recurrent units combined with a conditional random fields tagger gives the best results.

==> results_table_full.tex <==
\begin{table*}[!t]
\begin{tabularx}{\textwidth}{ |>{\hsize=0.58\hsize}X|>{\hsize=1.14\hsize}X|>{\hsize=1.14\hsize}X|>{\hsize=1.14\hsize}X| }
  \hline
   & Pointer Network & Neural CRF Tagger & Table Filling \\
  \hline 
  ATTN & 80.25; 70.12; 74.84; 88.62 & 77.29; \underline{73.19}; 75.18; \underline{89.15} & \underline{81.89}; 70.18; \underline{75.58}; 88.52\\
  (tuple level) & 75.50; 73.51; 74.49
 &  72.39; \underline{76.41}; 74.35
 & \underline{78.11}; 73.78; \underline{75.89} \\
    \hline 
CNN  & 82.72; \textbf{\underline{77.71}}; \textbf{\underline{80.14}}; \textbf{\underline{90.94}} & \textbf{\underline{86.25}}; 73.48; 79.35; 90.02 & \textbf{82.56}; 76.74; 79.54; 90.47\\
(tuple level)& 78.23; \textbf{\underline{80.62}}; \textbf{79.41} & \textbf{\underline{82.59}}; 76.84; 79.61 & \textbf{78.47}; 79.76; 79.11$^*$  \\
    \hline 
  RNN  & \textbf{82.94}; 76.19; 79.42; 90.91 & \underline{86.20}; \textbf{78.25}; \textbf{\underline{82.03}}; \textbf{\underline{91.55}} & 82.31; \textbf{\underline{78.38}}; \textbf{80.30}; \textbf{91.03}\\
(tuple level)& \textbf{78.80}; 79.17; 78.99 & \underline{82.53}; \textbf{81.19}; \textbf{\underline{81.86}} & 77.92; \textbf{\underline{81.44}}; \textbf{79.64}\\
  \hline
\end{tabularx}
\caption{Each cell contains seven evaluation measures: P/R/F/Acc on instance level, P/R/F on tuple
  level. The best values for each encoder (i.e., per row)
  are \underline{underlined}, the best values for each
  extractor (i.e., per column) are marked in \textbf{bold}.}
\label{tab:results}
\end{table*}
